A Comparative Study of How People With and Without ADHD Recognise and Avoid Dark Patterns on Social Media

Dark patterns are deceptive strategies that recent work in human-computer interaction (HCI) has captured throughout digital domains, including social networking sites (SNSs). While research has identified difficulties among people to recognise dark patterns effectively, few studies consider vulnerable populations and their experience in this regard, including people with attention deficit hyperactivity disorder (ADHD), who may be especially susceptible to attention-grabbing tricks. Based on an interactive web study with 135 participants, we investigate SNS users' ability to recognise and avoid dark patterns by comparing results from participants with and without ADHD. In line with prior work, we noticed overall low recognition of dark patterns with no significant differences between the two groups. Yet, ADHD individuals were able to avoid specific dark patterns more often. Our results advance previous work by understanding dark patterns in a realistic environment and offer insights into their effect on vulnerable populations.

==> tables/deceptive-strategy-recognition.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{p{0.12\textwidth} p{0.05\textwidth} p{0.05\textwidth} p{0.05\textwidth} p{0.05\textwidth}}
        \toprule
        \multicolumn{5}{c}{Dark Pattern} \\ \hline
        & Yes & Maybe & No & Total \\
        \midrule
        ADHD & 13 & 7 & 15 & 35 \\
        Non-ADHD & 7 & 8 & 19 & 34 \\
        \midrule
        \multicolumn{5}{c}{Non-Dark Pattern} \\ 
        \midrule
        & Yes & Maybe & No & Total \\
        \midrule
        ADHD & 6 & 6 & 21 & 33 \\
        Non-ADHD & 5 & 6 & 22 & 33 \\
        \bottomrule
    \end{tabular}
    \label{tab:deceptive-strategy-recognition}
\end{table}


==> tables/multi-anova-tables.tex <==

\begin{table*}[htb]
    \begin{minipage}[]{.475\textwidth}
        \resizebox{1\textwidth}{!}{
        \begin{tabular}{lcccc}
        \toprule
        &\multicolumn{4}{c}{\textbf{Factors}}\\\cmidrule{2-5}
        &\multicolumn{2}{c}{\textbf{\textsc{Task Version}}}&\multicolumn{2}{c}{\textbf{\textsc{Group Type}}}\\
        %\textbf{Response Variable} & \textsc{Task Version} $F(1, 114)=$  & \textsc{Task Version}  $p=$ &\textsc{Group Type} $F(1, 114)=$ & \textsc{Group Type} $p=$ \\
        %\textbf{Response Variable} & \textsc{Task Version} & \textsc{Task Version} & \textsc{Group Type} & \textsc{Group Type} \\
         & $F(1, 114)$  & $p$ & $F(1, 114)$ & $p$ \\

        \midrule
        %\textit{I1 -- Asymmetric (t1)} & 9.67 & \textbf{$<.01$} & 0.18 & 0.6693 \\
        \textit{I1 -- Asymmetric (t1)} & 9.67 & \textbf{<.01} & 0.18 & 0.669 \\
        \textit{I1 -- Asymmetric (t2)} & 0.05 & 0.821 & 0.07 & 0.793 \\
        \midrule
        %\textit{I2 -- Covert (t1)} & 15.89 &\textbf{ 0.0001***} & 1.45 & 0.2320 \\
        \textit{I2 -- Covert (t1)} & 15.89 &\textbf{ <.001} & 1.45 & 0.232 \\
        \textit{I2 -- Covert (t2)} & 0.29 & 0.592 & 3.29 & 0.073 \\
        \midrule
        %\textit{I3 -- Deceptive (t1)} & 7.75 & \textbf{0.0065**} & 0.01 & 0.9451 \\
        \textit{I3 -- Deceptive (t1)} & 7.75 & \textbf{<.01} & 0.01 & 0.945 \\
        \textit{I3 -- Deceptive (t2)} & 1.02 & 0.314 & 0.21 & 0.650 \\
        \midrule
        %\textit{I4 -- Disparate Treat. (t1)} & 9.07 & \textbf{0.0033** }& 0.01 & 0.9041 \\
        \textit{I4 -- Disparate Treat. (t1)} & 9.07 & \textbf{<.01 }& 0.01 & 0.904 \\
        \textit{I4 -- Disparate Treat. (t2)} & 0.00 & 0.995 & 0.30 & 0.5878 \\
        \midrule
        %\textit{I5 -- Hides Info. (t1)} & 17.52 & \textbf{0.0001***} & 0.22 & 0.6393 \\
        \textit{I5 -- Hides Info. (t1)} & 17.52 & \textbf{<.001} & 0.22 & 0.639 \\
        \textit{I5 -- Hides Info. (t2)} & 0.03 & 0.863 & 0.37 & 0.5469 \\
        \midrule
        %\textit{I6 -- Restrictive (t1)} & 27.00 &\textbf{ 1.11e-06***} & 0.21 & 0.6491 \\
        \textit{I6 -- Restrictive (t1)} & 27.00 &\textbf{<.001} & 0.21 & 0.649 \\
        \textit{I6 -- Restrictive (t2)} & 0.23 & 0.634 & 0.26 & 0.614 \\
        \midrule\midrule
        %\textit{I7 -- Definition} & 10.80 &\textbf{ 0.0012**} & 3.85 & 0.0523 \\
        \textit{I7 -- Definition} & 10.80 &\textbf{ <.01} & 3.85 & 0.052 \\
        %Task (Mixed) & 15.38 &\textbf{ 0.0002***} & - & - \\
        \bottomrule
    \end{tabular}
    }
    \caption{ART-ANOVA results for the presence of dark patterns in the UI as well as ADHD for participants for items I1-I7. the tasks, t1 = Task 1 and t2 = Task 2. Significant factors are highlighted by \textbf{bold} lettering. As we did not obtain any interaction effects between the factors for these items (p>.05), we do not report these measures in this table.}
    \label{tab:anova_i1-7}
    \end{minipage}
    \hfill
    \begin{minipage}[]{0.475\textwidth}
    \resizebox{1\textwidth}{!}{

        \begin{tabular}{lrcccc}
\toprule
\textbf{NASA TLX}  &    &&\\
\textbf{Subscale}  & \textbf{Factor}     & \textbf{F (1, 114)} & \textbf{$p$}\\
\midrule
\textbf{Effort}              & \textsc{Group Type}                                   & 7.97             & \textbf{0.005}         \\
                             & \textsc{Task Version}                         & 0.68             & 0.412            \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}             & 1.91             & 0.168            \\
\midrule
\textbf{Frustration}         & \textsc{Group Type}                                 & 5.03             & \textbf{0.026}          \\
                             & \textsc{Task Version}                        & 6.38             & \textbf{0.012}          \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}            & 0.02             & 0.879            \\
\midrule
\textbf{Mental}       & \textsc{Group Type}                                   & 1.65             & 0.201            \\
\textbf{Demand}                             & \textsc{Task Version}                          & 5.24             & \textbf{0.023   }         \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}           & 0.00             & 0.960            \\
\midrule
\textbf{Physical}     & \textsc{Group Type}                                 & 6.70             & \textbf{0.010  }          \\
\textbf{Demand}                             & \textsc{Task Version}                         & 1.48             & 0.226            \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}           & 0.00             & 0.974            \\
\midrule
\textbf{Performance}         & \textsc{Group Type}                                  & 0.12             & 0.725            \\
                             & \textsc{Task Version}                        & 1.65             & 0.200            \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}            & 0.93             & 0.337            \\
\midrule
\textbf{Temporal}     & \textsc{Group Type}                                  & 2.56             & 0.111            \\
\textbf{Demand}                             & \textsc{Task Version}                           & 2.76             & 0.098          \\
                             & \textsc{Group Type} $\times$ \textsc{Task Version}           & 0.06             & 0.809            \\
\bottomrule
\end{tabular}
}
\caption{ART-ANOVA results for the NASA-TLX with significant effects highlighted in bold.}
\label{tab:anova_nasa-tlx}
    \end{minipage}
\end{table*}

    

